A Simple Solution for Offline Imitation from Observations and Examples with Possibly Incomplete Trajectories

Offline imitation from observations aims to solve MDPs where only task-specific expert states and task-agnostic non-expert state-action pairs are available. Offline imitation is useful in real-world scenarios where arbitrary interactions are costly and expert actions are unavailable. The state-of-the-art "DIstribution Correction Estimation" (DICE) methods minimize divergence of state occupancy between expert and learner policies and retrieve a policy with weighted behavior cloning; however, their results are unstable when learning from incomplete trajectories, due to a non-robust optimization in the dual domain. To address the issue, in this paper, we propose Trajectory-Aware Imitation Learning from Observations (TAILO). TAILO uses a discounted sum along the future trajectory as the weight for weighted behavior cloning. The terms for the sum are scaled by the output of a discriminator, which aims to identify expert states. Despite simplicity, TAILO works well if there exist trajectories or segments of expert behavior in the task-agnostic data, a common assumption in prior work. In experiments across multiple testbeds, we find TAILO to be more robust and effective, particularly with incomplete trajectories.

==> Experiments_backup.tex <==
\section{Experiments}
\label{sec:experiment}
In this section, we evaluate  TAILO  on five different, challenging tasks across multiple mujoco testbeds. More specifically, we  study the following two questions: 1) Is the algorithm indeed robust to incomplete trajectories in either task-specific (Sec.~\ref{sec:incompleteTS}) or task-agnostic (Sec.~\ref{sec:incompleteTA}) data, and does it work with little expert data in the task-agnostic dataset (Sec.~\ref{sec:standard})? 2) Can the algorithm also work well in example-based IL (Sec.~\ref{sec:goal}) and learn from experts of different dynamics (Sec.~\ref{sec:mismatch})? %  which proves that it works better than SMODICE in all scenarios tested by the prior work? 

% Does the algorithm really succeed in discriminating expert and non-expert trajectories and segments in the task-agnostic data, and how important is our thresholding and PU learning design?  This problem is put into the appendix.

\textbf{Baselines.} We compare our method to four baselines: SMODICE~\cite{ma2022smodice}, LobsDICE~\cite{Kim2022LobsDICEOL}, ORIL~\cite{Zolna2020OfflineLF}, and plain behavior cloning (BC). Since LobsDICE works with state-pair occupancy, it cannot solve example-based IL; thus, we substitute LobsDICE in example-based IL with RCE~\cite{Eysenbach2021ReplacingRW}, a state-of-the-art online example-based RL method. Unless otherwise specified, we use 3 seeds for each method under each scenario. %We use the identical network architecture to that used in SMODICE~\cite{ma2022smodice}. ; for BC, we simply set all coefficient to $1$ and run our method.

\textbf{Environment Setup.} Following SMODICE~\cite{ma2022smodice}, unless otherwise specified, we test our algorithm on four standard mujoco testbeds from the OpenAI Gym~\cite{1606.01540}, which are the hopper, halfcheetah, ant and walker2d environment. We use normalized average reward\footnote{Normalization standard is according to D4RL~\cite{fu2020d4rl}, and  identical to SMODICE~\cite{ma2022smodice}.} as the main metric, where higher reward indicates better performance; for environments where the final reward is similar, fewer gradient steps in weighted behavior cloning indicates better performance. In this section, we use reward as criteria (higher is better; if the reward upon convergence is the same, fewer gradient steps to attain the reward indicates better convergence).
We report the change of the mean and standard deviation of reward with respect to the number of gradient steps.

\textbf{Experimental Setup.} For all environments, we use $\alpha=1.25, \beta_1=0.8,\eta_p=0.2$; $\beta_2=1$ if $D_{\text{TS}}$ and $D_{\text{TA}}$ are generated by different embodiments, and $\beta_2=0$ otherwise. 
%We use $\gamma=0.98$ for kitchen and pointmaze (see Sec.~\ref{sec:mismatch} for details), as expert episodes are shorter in these environments; 
We use $\gamma=0.998$ unless otherwise specified. We use an exactly identical discriminator and policy network as SMODICE: for the discriminator $c(s)$ and $c'(s)$, we use a small Multi-Layer Perceptron (MLP) with two hidden layers, width $256$, and tanh activation function. For actor $\pi$, we use an MLP with two hidden layers, width $256$, and ReLU~\cite{agarap2018deep} activation function. For the training of $c(s)$ and $c'(s)$, we use a learning rate of $3\times 10^{-4}$ and a 1-Lipschitz regularizer, run $10$K gradient steps for the training of $c'(s)$, and run $40$K gradient steps for the training of $c(s)$. For weighted behavior cloning, we use a learning rate of $10^{-4}$, a weight decay of $10^{-5}$, and run $1$M gradient steps. For discriminator training, we use a batch size of $512$; for weighted BC steps, we use a batch size of $8192$. Adam optimizer~\cite{Adam} is used for both steps. See Appendix~\ref{sec:addimp} for more details and Appendix~\ref{sec:addres} for a sensitivity analysis regarding the batch size, $\alpha, \beta_1, \beta_2, \eta_p$,  and $\gamma$.
% sensitivity analysis or ablation?
%TODO: add the value of gamma! need to count which one uses which. it is in {0.98, 0.998}. Also, do we need to mention that "large batch size does not help for the baselines" here?


\subsection{Standard Offline Imitation Learning from Observation}
\label{sec:standard}

\textbf{Environment Setup.} Besides the four standard mujoco environments specified above, we also test two more challenging environments, which are the Franka kitchen environment and the antmaze environment from D4RL~\cite{fu2020d4rl}. In the former, the agent needs to control a 9-DoF robot arm to complete a sequence of item manipulation subtasks, such as moving the kettle or opening the microwave; in the latter, the agent needs to control a robot ant to crawl through a U-shaped maze and get to a particular location. As kitchen environment requires less steps to finish, we use $\gamma=0.98$ instead of $0.998$.  

\textbf{Dataset Setup.} Following SMODICE~\cite{ma2022smodice}, for mujoco environments, we use offline datasets from D4RL~\cite{fu2020d4rl}, where a single trajectory from the ``expert-v2'' dataset is used as the task-specific data. The task-agnostic data consists of $40$ expert trajectories (about $40$K steps) from the ``expert-v2'' dataset and $1$M steps from the ``random-v2'' dataset. Note this setting contains $5\times$ fewer expert trajectories than SMODICE; see Appendix~\ref{sec:addres} for results with identical settings.
%which is 5x fewer than SMODICE.
For the kitchen and antmaze environment, we use the identical dataset as SMODICE, where a single trajectory is used as the task-specific dataset. The task-agnostic dataset for the kitchen environment consists of expert trajectories  completing different subtasks (both relevant and irrelevant) in different orders, and the task-agnostic dataset for antmaze consists of data with varied optimality. See Appendix \ref{sec:addimp} for more details.   

\begin{figure}
    \centering
\includegraphics[width=\linewidth]{pic/expert40/plot-expert40-May-2.png}
     \caption{Reward curves for standard offline imitation learning from observation, where the x-axis is the number of gradient steps and the y-axis is the normalized reward. In all six environments, our method either outperforms or is comparable to the baselines.}
    \label{fig:expert40}
\end{figure}

\textbf{Main Results.} Fig.~\ref{fig:expert40} shows the result for different methods in standard offline imitation learning from observations. We find our method to outperform all baselines on hopper, halfcheetah, ant and walker2d. Results are comparable to the best baseline on kitchen and antmaze. In the experiment, we found ORIL to often diverge, and the performance of SMODICE varies greatly depending on the $f$-divergence: on hopper, halfcheetah and walker2d, KL-divergence is much better, while $\chi^2$-divergence is better on ant and kitchen. LobsDICE is marginally better than SMODICE, as the former considers state-pair occupancy instead of single state, which is more informative. Also worth noting: none of the methods exceeds a normalized reward of $60$ in the kitchen environment; this is because the SMODICE experiment uses expert trajectories that are only expert for the first 2 out of all 4 subtasks. See Sec.~\ref{sec:kitcor} in the Appendix for a detailed discussion. 




% TODO: further beautify the figure!

\subsection{Offline Imitation Learning from Task-Agnostic Dataset with Incomplete Trajectories}
\label{sec:incompleteTA}

\textbf{Dataset Setup and Main Results.} We use the same task-specific dataset as in Sec.~\ref{sec:standard}. For the task-agnostic dataset, we iterate over the state-action pairs, and remove one pair for every $x$ pairs. In this work, we test $x\in\{2,3,5,10,20\}$. Fig.~\ref{fig:ta} shows the result for different methods with incomplete task-agnostic trajectories, where our method outperforms all baselines and remains largely stable despite decrease of $x$ (i.e., increase of removed data), as the coefficient for each state-action pair does not change much. In the training process, we often witness  SMODICE and LobsDICE to collapse due to diverging value functions (see Sec.~\ref{sec:dice} for explanation), which is expected; for runs that abort due to numerical error, we use a reward of $0$ for the rest of the gradient steps. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{pic/incompleteTA/plot-missing-May-2-small.png}
    \caption{Reward curves for offline imitation learning with incomplete trajectories in the task-agnostic dataset. The title for each subfigure is in the format of ``environment name''+``$1/x$'' (task-agnostic data removed), where $x\in\{2,3,5,10,20\}$. It is clearly illustrated that ours is the most stable method.
    }
    \label{fig:ta}
\end{figure}


\subsection{Offline Imitation Learning from Task-Specific Dataset with Incomplete Trajectories}
\label{sec:incompleteTS}
\textbf{Dataset Setup and Main Results.} We use the same task-agnostic dataset as in Sec.~\ref{sec:standard}. For the task-specific dataset, we only use the first $x$ steps and last $y$ steps in the expert trajectory, and discard the remainder. In this work, we test $(x,y)\in\{(1,100), (10,90), (50,50), (90,10) ,(100, 1)\}$. Fig.~\ref{fig:ts} shows the result for different methods with incomplete task-specific trajectories, where our method outperforms all baselines and often achieves results similar to those obtained when using the entire task-specific dataset. In contrast, SMODICE and LobsDICE are expectedly unstable in this setting.  

% TODO: ablation!
%Fig.~\ref{fig:ablate} shows the $R(s)$ and coefficient (normalized to 1) for each state-action pair along expert and non-expert trajectory with $(x,y)=(1,100)$ and $(x,y)=(100,1)$; in the former, 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{pic/incompleteTS/plot-ht-May-2-small.png}
    \caption{Reward curves for offline imitation with incomplete trajectories in the task-specific dataset. The title format for each subfigure is ``environment name''+``head $x$''+``tail $y$'' (states remained), where $(x,y)\in\{(100,1),(90,10),(50,50),(10,90),(1,100)\}$. It is clearly illustrated that ours is the most stable method.}
    \label{fig:ts}
\end{figure}

% TODO: ablation figure!

\subsection{Offline Imitation Learning from Examples}
\label{sec:goal}
\textbf{Environment Setup.} Following SMODICE, we test example-based offline imitation in three different testbeds: pointmaze, kitchen and antmaze. In the mujoco-based~\cite{todorov2012mujoco} pointmaze environment the agent needs to control a pointmass on a 2D plane to navigate to a particular direction. For the kitchen environment, we test two different settings where the agent is given successful examples of moving the kettle and opening the microwave respectively (denoted as ``kitchen-kettle'' and ``kitchen-microwave'').

\textbf{Dataset Setup.} Following SMODICE, we use a small set of success examples: hundreds of final states (see Appendix~\ref{sec:addimp} for details) are given as the task-specific dataset. For pointmaze, the task-agnostic data contains $60$K steps, generated by a script and distributed evenly along four directions (i.e., $25\%$ expert data); for other testbeds, the task-agnostic data is identical to the one discussed  in Sec.~\ref{sec:standard}.

\textbf{Main results.} Fig.~\ref{fig:goal} shows the results for offline imitation learning from examples on all environments tested in SMODICE; our simple method is marginally better than the baselines on pointmaze, antmaze and kitchen-microwave, and is comparable (all close to perfect) on kitchen-kettle. % The instability on the pointmaze environment is mainly because the trajectories in the task-agnostic dataset is too similar, i.e., only has little coverage of state space and thus make all algorithms more brittle.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{pic/goal/plot-goal-May-2.png}
    \caption{Reward curves for offline imitation learning from examples.}
    \label{fig:goal}
\end{figure}


\subsection{Offline Imitation Learning from Mismatched Dynamics}
\textbf{Environment and Dataset Setup.} Following SMODICE, we test our method on three environments: antmaze, halfcheetah and ant. We use task-specific data from an expert with different dynamics (e.g., halfcheetah with a shorter torso; see Sec.~\ref{sec:addexp} for details). Task-agnostic data follows Sec.~\ref{sec:standard}. % In antmaze environment, the agent needs to learn from a pointmass agent, where only the first two dimensions in state space indicating current coordinate is useful; in halfcheetah environment, the agent learns from a halfcheetah with much shorter torso; in ant environment, the agent learns from an expert with one leg crippled. Due to large variance, we run 10 seeds instead of 3 for this experiment.

\textbf{Main Results.} Fig.~\ref{fig:mismatch} shows the results for offline imitation learning from mismatched dynamics, where our method is the best in all three testbeds. Among the three environments, halfcheetah is the most difficult, as the state space for halfcheetah with shorter torso is unreachable by a normal halfcheetah, i.e., the assumption that $d^{\text{TA}}(s)>0$ wherever $d^{\text{TS}}(s)>0$ in SMODICE and LobsDICE does not hold; in such a setting, our method is much more robust than DICE methods.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{pic/mismatch/plot-mismatch-May-2.png}
    \caption{Reward curves for offline imitation learning from mismatched dynamics.}
    \label{fig:mismatch}
\end{figure}

\label{sec:mismatch}
% emphasize the "incomplete" part; go into the title, and elaborate why better working with inocmplete expert demonstrations 
% guide with "dealing with incomplete demonstrations"
% why existing works struggle with incomplete demonstrations 
% "examples" in the related work session / discussion session 
% explain the difference between "examples" and "incomplete trajectories"
% possibly incomplete


% {
% \begingroup
% \begin{figure}[t]
% \begin{minipage}[c]{0.32\linewidth}
% \subfigure[Hopper]{\includegraphics[width=\linewidth]{pic/normal/plot-hopper-normal-Mar.jpg}}
% %\subcaption*{\scalebox{0.85}{a) Kitchen-SKiLD-A}}
% \subfigure[HalfCheetah]{\includegraphics[width=\linewidth]{pic/normal/plot-ant-normal-Mar.jpg}}
% %\subcaption*{\scalebox{0.85}{d) Kitchen-FIST-B}}
% \end{minipage}
% \begin{minipage}[c]{0.32\linewidth}
% \subfigure[Ant]{\includegraphics[width=\linewidth]{pic/normal/plot-halfcheetah-normal-Mar.jpg}}
% \subfigure[Walker2d]{\includegraphics[width=\linewidth]{pic/normal/plot-walker2d-normal-Mar.jpg}}

% \end{minipage}
% \begin{minipage}[c]{0.32\linewidth}

% \subfigure[Kitchen]{\includegraphics[width=\linewidth]{pic/normal/plot-kitchen-normal-Mar.jpg}}
% \subfigure[Antmaze]{\includegraphics[width=\linewidth]{pic/normal/plot-antmaze-normal-Mar.jpg}}

% %\caption*{Kitchen-FIST-}
% %\input{pic/new198/new infection prop}
% \end{minipage}
% \begin{minipage}[c]{0.24\linewidth}
% % \includegraphics[width=\linewidth]{pic/spread/corner_10.pdf}
% % \caption*{\scalebox{0.8}{d) 10d from corner}}
% \end{minipage}
% \caption{Normal}
% %\vspace{-15pt}
% \label{fig:normal}
% \end{figure}
% \endgroup
% }

% \begin{figure}[t]
%     \centering
%     \subfigure[Hopper]{ % this figure is retrieved from google picture
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/expert40/plot-hopper-expert40-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[HalfCheetah]{
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/expert40/plot-halfcheetah-expert40-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[Ant]{ % this figure is retrieved from google picture
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/expert40/plot-ant-expert40-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[Walker2d]{
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/expert40/plot-walker2d-expert40-Mar.jpg}
%     \end{minipage}
%     }
%     \caption{only use 40 expert trajectories in TA}
%     \label{fig:expert40}
% \end{figure}

% including normal dataset / less expert trajectory
% #seed * #scenario * #BS * #f (KL/chi)
% ours: #seed * (2 + 4 * 2) = 10 * #seed
% lobsdice: #seed * (2 + 4 * 2) * 2 = 20 * #seed
% smodice: #seed * (2 + 4 * 2) * 2 * 2 = 40 * #seed
% other baselines: #seed * (2 + 4 * 2) * 2 = 20 * #seed * #method




% first 1 / 10 / 50 / 90 / 100 step(s) + last 100 / 90 / 50 / 10 / 1 step(s)
% #seed * #scenario * #BS * #f (KL/chi)
% ours: #seed * (4 * 5) = 20 * #seed
% lobsdice: #seed * (4 * 5) * 2 = 40 * #seed
% smodice: #seed * (4 * 5) * 2 * 2 = 80 * #seed
% other baselines: #seed * (4 * 5) * 2 = 40 * #seed * #method

% \begin{figure}[t]
%     \centering
%     \subfigure[Hopper]{ % this figure is retrieved from google picture
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/h0.1t0.001/plot-hopper-h0.1t0.001-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[HalfCheetah]{
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/h0.1t0.001/plot-halfcheetah-h0.1t0.001-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[Ant]{ % this figure is retrieved from google picture
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/h0.1t0.001/plot-ant-h0.1t0.001-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[Walker2d]{
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/h0.1t0.001/plot-walker2d-h0.1t0.001-Mar.jpg}
%     \end{minipage}
%     }
%     \caption{only use first 100 step and last 1 step in TS}
%     \label{fig:h0.1t0.001}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \subfigure[Hopper]{ % this figure is retrieved from google picture
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/h0.09t0.01/plot-hopper-h0.09t0.01-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[HalfCheetah]{
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/h0.09t0.01/plot-halfcheetah-h0.09t0.01-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[Ant]{ % this figure is retrieved from google picture
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/h0.09t0.01/plot-ant-h0.09t0.01-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[Walker2d]{
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/h0.09t0.01/plot-walker2d-h0.09t0.01-Mar.jpg}
%     \end{minipage}
%     }
%     \caption{only use first 90 step and last 10 step in TS}
%     \label{fig:h0.09t0.01}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \subfigure[Hopper]{ % this figure is retrieved from google picture
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/h0.05t0.05/plot-hopper-h0.05t0.05-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[HalfCheetah]{
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/h0.05t0.05/plot-halfcheetah-h0.05t0.05-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[Ant]{ % this figure is retrieved from google picture
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/h0.05t0.05/plot-ant-h0.05t0.05-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[Walker2d]{
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/h0.05t0.05/plot-walker2d-h0.05t0.05-Mar.jpg}
%     \end{minipage}
%     }
%     \caption{only use first 50 step and last 50 step in TS}
%     \label{fig:h0.05t0.05}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \subfigure[Hopper]{ % this figure is retrieved from google picture
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/h0.01t0.09/plot-hopper-h0.01t0.09-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[HalfCheetah]{
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/h0.01t0.09/plot-halfcheetah-h0.01t0.09-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[Ant]{ % this figure is retrieved from google picture
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/h0.01t0.09/plot-ant-h0.01t0.09-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[Walker2d]{
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/h0.01t0.09/plot-walker2d-h0.01t0.09-Mar.jpg}
%     \end{minipage}
%     }
%     \caption{only use first 10 step and last 90 step in TS}
%     \label{fig:h0.01t0.09}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \subfigure[Hopper]{ % this figure is retrieved from google picture
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{example-image-a}
%     \end{minipage}
%     }
%     \subfigure[HalfCheetah]{
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{example-image-a}
%     \end{minipage}
%     }
%     \subfigure[Ant]{ % this figure is retrieved from google picture
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{example-image-a}
%     \end{minipage}
%     }
%     \subfigure[Walker2d]{
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{example-image-a}
%     \end{minipage}
%     }
%     \caption{only use first 1 step and last 100 step in TS}
%     \label{fig:h0.001t0.1}
% \end{figure}



% remove every 20 / 10 / 5 / 3 / 2 step in the TA dataset; DICE method does not work well with TA steps missing
% ours: #seed * (4 * 5) = 20 * #seed
% lobsdice: #seed * (4 * 5) * 2 = 40 * #seed
% smodice: #seed * (4 * 5) * 2 * 2 = 80 * #seed
% other baselines: #seed * (4 * 5) * 2 = 40 * #seed * #method 

% remove step without dealing with next state?

% \begin{figure}[t]
%     \centering
%     \subfigure[Hopper]{ % this figure is retrieved from google picture
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/missing20/plot-hopper-missing20-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[HalfCheetah]{
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/missing20/plot-halfcheetah-missing20-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[Ant]{ % this figure is retrieved from google picture
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/missing20/plot-ant-missing20-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[Walker2d]{
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/missing20/plot-walker2d-missing20-Mar.jpg}
%     \end{minipage}
%     }
%     \caption{Every 20 step is missing in TA}
%     \label{fig:miss20}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \subfigure[Hopper]{ % this figure is retrieved from google picture
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/missing10/plot-hopper-missing10-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[HalfCheetah]{
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/missing10/plot-halfcheetah-missing10-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[Ant]{ % this figure is retrieved from google picture
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/missing10/plot-ant-missing10-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[Walker2d]{
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/missing10/plot-walker2d-missing10-Mar.jpg}
%     \end{minipage}
%     }
%     \caption{Every 10 step is missing in TA}
%     \label{fig:miss10}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \subfigure[Hopper]{ % this figure is retrieved from google picture
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/missing5/plot-hopper-missing5-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[HalfCheetah]{
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/missing5/plot-halfcheetah-missing5-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[Ant]{ % this figure is retrieved from google picture
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/missing5/plot-ant-missing5-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[Walker2d]{
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/missing5/plot-walker2d-missing5-Mar.jpg}
%     \end{minipage}
%     }
%     \caption{Every 5 step is missing in TA}
%     \label{fig:miss5}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \subfigure[Hopper]{ % this figure is retrieved from google picture
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/missing3/plot-hopper-missing3-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[HalfCheetah]{
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/missing3/plot-halfcheetah-missing3-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[Ant]{ % this figure is retrieved from google picture
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/missing3/plot-ant-missing3-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[Walker2d]{
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/missing3/plot-walker2d-missing3-Mar.jpg}
%     \end{minipage}
%     }
%     \caption{Every 3 step is missing in TA}
%     \label{fig:miss3}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \subfigure[Hopper]{ % this figure is retrieved from google picture
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/missing2/plot-hopper-missing2-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[HalfCheetah]{
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/missing2/plot-halfcheetah-missing2-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[Ant]{ % this figure is retrieved from google picture
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/missing2/plot-ant-missing2-Mar.jpg}
%     \end{minipage}
%     }
%     \subfigure[Walker2d]{
%     \begin{minipage}[b]{0.23\linewidth}
%     \includegraphics[width=\linewidth]{pic/missing2/plot-walker2d-missing2-Mar.jpg}
%     \end{minipage}
%     }
%     \caption{Every 2 step is missing in TA}
%     \label{fig:miss2}
% \end{figure}


% ours: #seed * 4 = 2 * #seed
% smodice: #seed * 2 * 2 * 4 = 16 * #seed
% other baselines: #seed * 2 * 4 = 8 * #seed * #method 

% total: (70 + 140 + 140 + 18 + 108 * #method) * #seed = (368 + 108 * #method) * #seed 

% assume 20 runs per 6h / 80 runs per day (almost exclusive on az2, az4, az5)
% #seed = (5 - 1) = 4 (one already completed), #method = 2: 584 / 20 = 29.2 days

% from SMODICE; 300 goal state as task-speicific dataset


% run multiple times for the most crucial experiments; include explanation for running multiple seeds are expensive
%　convince people that the comparison is fair
% less seeds for secondary experiments

==> rebuttal.tex <==

% \begin{table}
% \begin{tabular}{c|ccccccc}
%    \hline
%    Dataset  & MOReL & MOPO & CQL & IQL & DT & 10\%BC & TAILO (ours) \\
%    \hline
%    halfcheetah-medium-v2 & 42.1 & 42.3  & 44.0 & 47.4 & 42.6 & 42.5 & 39.8 \\
%    hopper-medium-v2 & 95.4 & 28.0 & 58.5 & 66.3 & 67.6 & 56.9 & 56.2\\
%    walker2d-medium-v2 & 77.8 & 17.8 & 72.5 & 78.3 & 74.0 & 75.0 & 71.7\\
%    halfcheetah-medium-replay-v2 & 40.2 & 53.1 & 45.5 & 44.2 & 36.6 & 40.6 & 42.8\\
%    hopper-medium-replay-v2 & 93.6 & 67.5 & 95.0 & 94.7 & 82.7 & 75.9 & 83.4 \\
%    walker2d-medium-replay-v2 & 49.8 & 39.0 & 77.2 & 73.9 & 66.6 & 62.5 & 61.2 \\
%    halfcheetah-medium-expert-v2 & 53.3 & 63.3 & 91.6 & 86.7 & 86.8 & 92.9 & 94.3 \\
%    hopper-medium-expert-v2 & 108.7 & 23.7 & 105.4 & 91.5 & 107.6 & 110.9 & 111.5 \\
%    walker2d-medium-expert-v2 & 95.6 & 44.6 & 108.8 & 109.6 & 108.1 & 109.0 & 108.2 \\
%    \hline
%    Average & 72.9 & 42.1  & 77.6 & 77.0 & 74.7 & 74.0 & 74.3 \\
%    \hline
% \end{tabular}
% \caption{Comparison to offline RL methods (model-based and model-free) on standard D4RL environments. We adopt the results from ReCOIL and MOReL for the baselines. The best trajectory in the dataset is used as the task-specific dataset. Even if our method has no access to ground truth reward label and does not use expert action, it is still comparable to strong offline RL baselines.}
% \end{table}
% Note the comparison is favorable to other methods as we only know one expert trajectory in the dataset without access to ground-truth reward labels

\begin{figure}[h]
    \centering
    \subfigure[SMODICE (Sec.~\ref{sec:identical})  setting]{ % this figure is retrieved from google picture
    \begin{minipage}[b]{\linewidth}
    \includegraphics[width=0.85\linewidth]{plot-DWBC-OTR-MARWIL-normal.png}
    \end{minipage}
    }
    \subfigure[Sec.~\ref{sec:standard} setting]{
    \begin{minipage}[b]{\linewidth}
    \includegraphics[width=0.85\linewidth]{plot-DWBC-OTR-MARWIL-E40.png}
    \end{minipage}
    }
    
    
    \caption{Comparison to DWBC (with expert action), OTR, MARWIL (single-iteration AWR), ours with no positive-unlabeled learning (no PU) and $\gamma=0$. We found that both DWBC and OTR are not good at handling task-agnostic dataset with small portion of expert data. MARWIL performs similarly to plain BC, which is consistent with the findings from prior work. Our method with no PU generally works well, but $\gamma=0$ fails on many environments. \textbf{(For reviewer iGFb Q3, Q4; reviewer 6nYj Q3, Q5; reviewer Re2g Q2, Q6)}}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{plot-ablatePUgamma.png}
    \caption{Examples of failing cases of our method with no positive-unlabeled learning and $\gamma=0$. \textbf{(For reviewer iGFb Q4; reviewer 6nYj Q1; reviewer Re2g Q6)}}
    \label{fig:enter-label}
\end{figure}
% remove the table
% shorten the response
% 
% 
